Vorstellung eines sozioinformatischen Analyseansatzes zur Technikfolgenabsch\"atzung in Anlehnung an Vesters Sensitivit\"atsmodell am Beispiel des Unternehmens Uber als sozio-technisches System

What fits the human brain does not necessarily mean whatever is invented is meant for human brain. This is exactly what is implied by the definition of algorithm: \textit{Reducing and Simplifying}. Our cognitive apparatus, although endowed with certain parameters, ceases to comprehend chains of mathematical and logical steps used for algorithmic or mathematical purposes. Such a cognitive limit allows us to pay attention to the symbolic regularities which are meaningful. The more meaningless these symbols become, the fuzzier is our mental representation for it. Needless to say, that we actually tend to interact with activities that are meaningful, and discard those that are meaningless. By activities we mean steps, steps that form an algorithm. Could it be just an assumption? Are we really aversing from algorithms in modern day life? -- Ziel dieser Arbeit war eine kritische Auseinandersetzung mit dem biokybernetischen Denkansatz anhand des Sensitivit\"atsmodells von Frederic Vester, das in die sozioinformatische Analyse eines sozio-technischen Systems integriert und hinsichtlich der Fragestellung gepr\"uft wurde, inwieweit sich dieses Konzept zur Beurteilung von Planungsvorhaben bei sozio-technischen Systemen eignet. Dazu wurden F. Vesters Biokybernetischenn Grundregeln zur Feststellung der \"Uberlebensf\"ahigkeit eines Systems, auf ihre Anwendbarkeit in Bezug auf sozio-technische Systeme untersucht. Die Funktionalit\"at der Analysemethode wurde auf das nach der Definition von Andrea Kienle und Gabriele Kunau als sozio-technisches System charakterisierte Unternehmen Uber angewendet. Im Gegensatz zu unsystemischen Analysen besteht der Vorteil des Sensitivit\"atsmodells in der Vermittlung von Erkenntnissen \"uber innere Systemzusammenh\"ange. Abschlie{\ss}end wurde der vorgestellte Analyseansatz als transdisziplin\"are Weiterentwicklung des Sensitivit\"atsmodells charakterisiert.

==> anhang/anhang.tex <==
\subsection*{Anhang}\label{anhang}


==> latex_einstellungen/abkuezungen/abkuerzungen.tex <==
\nomenclature{UGC}{User Generated Content}
\nomenclature{CSS}{Cascading Style Sheets}
\nomenclature{JS}{JavaScript}
\nomenclature{SQL}{Structured Query Language}
\nomenclature{GPL}{GNU General Public License}
\nomenclature{GNU}{GNU is not Unix}
\nomenclature{LGPL}{GNU Lesser General Public License}
\nomenclature{XMPP}{Extensible Messaging and Presence Protocol}
\nomenclature{IM}{Instant Message}
\nomenclature{CMS}{Content Management System}
\nomenclature{RSS}{Really Simple Syndication}
\nomenclature{JSON}{JavaScript Object Notation}
\nomenclature{HTML}{Hypertext Markup Language}
\nomenclature{TDD}{Test-driven development}
\nomenclature{GUI}{Graphical User Interface}
\nomenclature{KPI}{Key Performance Indicator}
\nomenclature{WWW}{World Wide Web}
\nomenclature{OCR}{Optical Character Recognition}
\nomenclature{ERM}{Entity Relationship Modell}


==> sperrvermerk.tex <==
\section*{Sperrvermerk}
\textcolor{red}{
Die vorliegende Arbeit beinhaltet interne und vertrauliche Informationen der Firma <Firmenname>.
Die Weitergabe des Inhalts der Arbeit im Gesamten oder in Teilen sowie das Anfertigen
von Kopien oder Abschriften - auch in digitaler Form - sind grundsätzlich untersagt.
Ausnahmen bedürfen der schriftlichen Genehmigung der Firma <Firmenname>.
}
